Orientation Keypoints for 6D Human Pose Estimation

Most realtime human pose estimation approaches are based on detecting joint positions. Using the detected joint positions, the yaw and pitch of the limbs can be computed. However, the roll along the limb, which is critical for application such as sports analysis and computer animation, cannot be computed as this axis of rotation remains unobserved. In this paper we therefore introduce orientation keypoints, a novel approach for estimating the full position and rotation of skeletal joints, using only single-frame RGB images. Inspired by how motion-capture systems use a set of point markers to estimate full bone rotations, our method uses virtual markers to generate sufficient information to accurately infer rotations with simple post processing. The rotation predictions improve upon the best reported mean error for joint angles by 48% and achieves 93% accuracy across 15 bone rotations. The method also improves the current state-of-the-art results for joint positions by 14% as measured by MPJPE on the principle dataset, and generalizes well to in-the-wild datasets.

==> scrap2.tex <==

(densepose) [martin@bigboy crosshair]$ python scen_v8k21hr.py -m eval -i cr_v8k21hr_vox -c 0 -freq 13
Using VOXEL depth
Missing keys: []
extra keys: []
procrustes loss set to absolute - no z expansion
Finetuning 4 layers into the backbone
using device: cuda:0
Missing keys: []
loaded cr_v8k21hr_vox after epoch 36 with loss [0.13491496443748474, 0.015755264088511467, 0.02818949520587921, 0.0005635279230773449, 0.016907596960663795, 0.017877263948321342, 0.023482635617256165, 0.032139189541339874, 0.023129915818572044]
[('S9', 63596), ('S11', 46271)]
Dataset length: 8452
8 6 0
no lower 0.03419114
no upper 0.03430743
Showing main errors for k17 only, not k21.
extra joints [61.05985628 45.36579685 61.65019354 66.44753038] [0.23434984 0.27365783 0.57219911 0.60968506]
Mean 3d distance = 6.91% scrn. jkps=6.19
------------------------------------------------------------------
Pckh 0.9834
Mean distance = 4.27% scrn. jkps=3.40% scrn. okps=4.50.
Distance by kps
[2.43 3.27 2.87 3.73 3.6  3.19 3.53 3.98 3.67 2.71 2.46 2.17 1.66 2.93 3.   4.29 6.12 2.69 3.18 4.41 6.22]
[5.62 5.36 5.69 7.18 4.99 5.43 4.22 5.36 5.07 5.98 4.77 6.92 4.83 4.07 3.91 4.3  4.84 5.34 4.67 4.45 5.07 6.12 4.84
 5.71 5.38 4.78 4.5  4.38 2.34 3.29 2.69 3.03 3.12 2.45 3.07 4.04 2.79 2.94 3.3  3.44 2.18 2.47 2.34 2.07 2.87 4.09
 4.08 3.61 4.22 3.73 4.22 4.43 4.52 3.94 3.63 5.05 7.2  7.   6.57 7.42 3.29 4.75 3.93 3.29 4.2  3.84 4.02 4.33 4.63
 3.97 3.72 5.3  7.52 7.21 6.79 7.74]
3d distance by kps
[ 0.   17.22 43.05 61.06 17.22 45.37 69.54 33.67 37.47 51.71 53.23 51.04 61.65 76.88 46.94 66.45 81.7 ]
camera rotation error by joint
[0.145 0.226 0.246 0.192 0.229 0.144 0.149 0.31  0.179 0.188 0.226 0.26  0.232 0.226 0.268]
[0.145 0.22  0.147 0.253 0.142 0.179 0.2   0.308 0.331 0.216 0.388 0.177 0.237 0.392 0.184]
[[ 2.    3.    4.    5.    6.   12.    7.    8.    9.   10.   11.   13.   14.   15.   16.    0.  ]
 [ 3.04  3.71  3.27  5.51  4.14  3.71  2.94  3.72  5.2   9.42  4.01  5.69  2.83  4.08  2.73  4.27]
 [ 2.18  2.74  2.64  4.74  3.33  2.81  1.97  2.79  4.31  8.43  3.12  4.94  2.06  3.02  1.98  3.4 ]
 [ 3.28  3.97  3.44  5.72  4.37  3.96  3.21  3.98  5.45  9.69  4.26  5.9   3.04  4.37  2.93  4.5 ]
 [ 2.    2.49  2.12  4.61  2.51  2.45  1.97  2.33  3.09  7.49  2.54  4.61  1.89  2.73  1.75  2.97]
 [ 1.84  2.19  2.01  1.93  2.72  2.24  1.75  2.38  3.48  3.83  2.54  2.19  1.68  2.42  1.7   2.33]
 [ 3.52  4.67  4.24  3.89  4.62  4.81  3.53  4.53  6.11  7.22  4.66  3.97  3.18  5.06  3.28  4.49]
 [ 5.13  6.58  5.9   7.6   6.88  6.68  5.08  6.43  8.86 13.37  6.79  7.81  4.68  7.16  4.69  6.91]
 [ 4.35  5.75  5.49  6.89  6.23  6.    4.2   5.65  8.15 12.63  6.11  7.08  3.94  6.3   4.1   6.19]
 [44.37 48.87 42.64 45.46 49.77 50.93 43.01 44.41 56.64 62.31 48.27 44.06 38.79 49.51 42.12 47.41]
 [33.32 36.34 34.25 35.22 36.3  38.59 32.5  32.81 42.86 50.33 36.49 33.41 29.85 37.22 32.14 36.11]]
[[0.289 0.294 0.252 0.305 0.301 0.308 0.298 0.262 0.327 0.354 0.296 0.291 0.266 0.308 0.245 0.293]
 [0.216 0.218 0.177 0.224 0.21  0.227 0.202 0.189 0.249 0.251 0.217 0.213 0.186 0.233 0.186 0.213]
 [0.267 0.227 0.204 0.219 0.228 0.224 0.213 0.217 0.292 0.287 0.233 0.23  0.198 0.258 0.212 0.234]]


(densepose) [martin@bigboy lift]$  python scen_v1h21.py -m eval -la cr_v8k21hr_vox -c 0 -i lift_hr21_vox_l1_best -freq 1
Using VOXEL depth
procrustes loss set to absolute - no z expansion
Lin size: 1536 Res blocks: 2 Num dims: 3
>>> total params: 10.35M
using device: cuda:0
Missing keys: []
loaded lift_hr21_vox_l1_best after epoch 58 with loss [0.22183266282081604]
Using 97 inputs
Dataset length: 8452
Showing main errors for k17 only, not k21.
/home/martin/.conda/envs/densepose/lib/python3.7/site-packages/numpy/core/fromnumeric.py:3118: RuntimeWarning: Mean of empty slice.
  out=out, **kwargs)
/home/martin/.conda/envs/densepose/lib/python3.7/site-packages/numpy/core/_methods.py:85: RuntimeWarning: invalid value encountered in double_scalars
  ret = ret.dtype.type(ret / rcount)
Mean distance = 44.60mm. jkps=44.60mm. okps=nan.
Distance by kps
[ 0.2  21.43 45.36 62.74 21.47 42.77 69.4  34.5  34.39 44.53 48.81 44.37 54.6  69.95 42.24 58.34 73.78]
[]
[0.151 0.247 0.258 0.197 0.226 0.155 0.145 0.308 0.24  0.2   0.242 0.269 0.241 0.23  0.27 ]
[[ 2.   3.   4.   5.   6.  12.   7.   8.   9.  10.  11.  13.  14.  15.  16.   0. ]
 [40.7 45.5 39.5 42.3 48.1 49.2 40.3 39.6 56.7 61.3 45.8 41.2 35.3 46.8 36.8 44.6]
 [40.7 45.5 39.5 42.3 48.1 49.2 40.3 39.6 56.7 61.3 45.8 41.2 35.3 46.8 36.8 44.6]
 [ nan  nan  nan  nan  nan  nan  nan  nan  nan  nan  nan  nan  nan  nan  nan  nan]
 [31.7 34.5 32.7 33.9 35.4 38.1 31.5 30.9 42.9 49.2 35.8 32.3 27.6 35.8 30.5 34.9]
 [31.7 34.5 32.7 33.9 35.4 38.1 31.5 30.9 42.9 49.2 35.8 32.3 27.6 35.8 30.5 34.9]
 [ nan  nan  nan  nan  nan  nan  nan  nan  nan  nan  nan  nan  nan  nan  nan  nan]
 [43.9 48.1 41.7 45.3 51.  51.7 43.6 42.3 58.6 62.6 48.5 44.3 37.2 48.4 41.2 47.2]
 [32.7 35.4 33.6 35.4 36.9 39.6 33.6 32.  43.8 51.  36.7 33.7 28.7 36.4 32.6 36.1]]
[[0.223 0.231 0.18  0.229 0.228 0.236 0.218 0.19  0.27  0.268 0.233 0.222 0.19  0.238 0.188 0.223]
 [0.263 0.238 0.2   0.221 0.232 0.227 0.225 0.211 0.302 0.295 0.243 0.236 0.202 0.255 0.216 0.238]]


==> tables/ablation_table.tex <==
\begin{table*}[b!]
\centering

\caption{Results for different detectors, experiments on resolution, number of crosshairs for XY detections, second-stage refinement and training with feet/hands included (for comparability, averages in last scenario only includes 17 joints and 15 rotations)}

\begin{tabular}{lccc}\hline
 & \textbf{MPJAS} & \multicolumn{2}{c}\textbf{MPJPE-17} \\
 &(15 rot)   & \textbf{P1} & \textbf{P2} \\ \hline
\textit{256x192 Crosshairs (trained on 17j, 15r)} \\
Detector to skeleton (1-layer XY) & 0.239 & 52.2  & 39.6  \\
Detector to skeleton (4-layer XY) & 0.235 & 51.9  & 39.1  \\
Refined detections & NA & 49.2  & 38.0  \\
\hline
\textit{384x288 Crosshairs (trained on 17j, 15r)}  \\
Detector to skeleton (1-layer XY) & 0.217 & 48.1 & 37.2  \\
Detector to skeleton (4-layer XY) & 0.217 & 48.2 & 37.1 \\
Refined detections & NA  & 45.5 & 35.8 \\
\hline
\textit{384x288 Regression Detector (trained on 17j, 15r)}  \\
Detector to skeleton  & 0.228 & 52.4 & 40.6  \\
Refined detections & NA  & 51.6 & 37.3 \\

\hline
\textit{384x288 Crosshairs (trained on 21j, 19r)} &  &  &  \\
Detector to skeleton (1-layer XY) & 0.216 & 47.8 & 36.7  \\
Detector to skeleton (4-layer XY) & \textbf{0.213} & 47.4 & 36.1 \\
Refined detections & NA  &\textbf{44.6}  &\textbf{34.9}  \\
\hline
\\
\end{tabular}

\label{tab:ablation}
\end{table*}

==> tables/ablation_table_old.tex <==
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}\hline
 & \textbf{MPJAS} & \multicolumn{2}{c}\textbf{MPJPE-17} \\
 &(15 rot)   & \textbf{P1} & \textbf{P2} \\ \hline
\textit{256x192 Crosshairs} &  &  &  \\
Detector to skeleton (1-layer XY) & 0.243 & 51.7  & 40.3  \\
Detector to skeleton (4-layer XY) & 0.239 & 51.7  & 39.8  \\
Refined detections & NA & 49.2  & 38.0  \\
Refined to skeleton & 0.243 &50.4  &39.2  \\
\hline
\textit{384x288 Crosshairs (trained on 17j, 15r)}  \\
Detector to skeleton (1-layer XY) & 0.221 & 48.6 & 37.9  \\
Detector to skeleton (4-layer XY) & 0.220 & 48.7 & 37.8 \\
Refined detections & NA  & 45.5 & 35.8 \\
Refined to skeleton & 0.227 & 47.5  & 37.0 \\
\hline
\textit{384x288 Crosshairs (trained on 21j, 19r)} &  &  &  \\
Detector to skeleton (1-layer XY) & 0.220 & 48.0 & 37.6  \\
Detector to skeleton (4-layer XY) & \textbf{0.217} & 47.9 & 37.1 \\
Refined detections & NA  &\textbf{44.9}  &\textbf{35.5}  \\
Refined to skeleton &0.224  &  46.9 & 36.6  \\

\hline
\end{tabular}

}

\caption{Results for different experiments on resolution, number of crosshairs for XY detections, second-stage refinement and training with feet/hands included (results for last scenario only includes 17 joints and 15 rotations)}
\label{tab:ablation}
\end{table}

==> tables/gt_table.tex <==
\begin{table*}[t!]
\centering
\caption{Ground truth trained MPJPE using 2D keypoints (no depth info), with/without a set of 2 orientation keypoints per joint. For video we use 9 frames, each spaced 5 frames apart}


\begin{tabular}{lrrr}
\hline
\multicolumn{1}{c}{}    & Only      & With      &  \\ 
                        & JKPS      & OKPS      & $\Delta$ \\ \hline
\textit{Protocol 1 - MPJPE mm}    &           &           &          \\
GT / GT Single Frame  \\
Martinez \etal \cite{martinez_2017_3dbaseline} & 45.5     &      \\
Orientation keypoints (ours)    & 48.3     &\textbf{33.3}     &\textit{(-31\%)} \\ \hline
GT / GT Video  \\
Pavllo \etal \cite{DBLP:PavLLO_3Dhumanposeinvideo} 243 frame & 37.2  & & \\
Orientation keypoints (ours)  9x1:5 frame   &       &\textbf{28.8} &   \\ \hline \hline

\textit{Protocol 2 (Procrustes) - MPJPE mm} &  &                    \\
GT / GT Single Frame  \\
Martinez \etal \cite{martinez_2017_3dbaseline} & 37.1 &   \\
Orientation keypoints (ours)    & 34.9     & \textbf{24.9}      &\textit{(-29\%)}    \\ \hline
GT / GT Video  \\
Pavllo \etal \cite{DBLP:PavLLO_3Dhumanposeinvideo} 243 frame & 27.2  & &  \\
Orientation keypoints (ours) 9x1:5 frame &      & \textbf{20.1}     &     \\ \hline \hline
\textit{Rotation error - MPJAS-15 radians} &  &          \\
OKPS single frame (ours)    &      & \textbf{0.150} &  \\
OKPS video (ours) 9x1:5 frame  &      & \textbf{0.106} &\\ \hline
\hline\\
\end{tabular}


\label{tab:gt_table}
\end{table*}

==> tables/mpjpe_table_imp.tex <==
\begin{table*}[]
\centering
\resizebox{0.99\textwidth}{!}{%

\begin{tabular}{lrrrrrrrrrrrrrrr|r}
\hline
\textbf{Protocol \#1} & Dir & Disc & Eat & Greet & Phone & Photo & Pose & Punch & Sit & SitD & Smoke & Wait & WalkD & Walk & WalkT & Avg \\ \hline
\multicolumn{1}{l|}{Zhou \etal~\cite{DBLP:journals/corr/Zhou0ZLW16} ECCV '16} & 91.8 & 102.4 & 97.0 & 98.8 & 113.3 & 125.2 & 90.0 & 93.8 & 132.2 & 159.0 & 106.9 & 94.4 & 126.0 & 79.0 & 99.0 & 107.3 \\
\multicolumn{1}{l|}{Moreno-Noguer \cite{Moreno-Noguer_2017_CVPR} CVPR '17}
& 66.1 & 61.7 & 84.5 & 73.7 & 65.2 & 67.2 & 60.9 & 67.3 & 103.5 & 74.6 & 92.6 & 69.6 & 71.5 & 78.0 & 73.2 & 74.0 \\ 
\multicolumn{1}{l|}{Pavlakos \etal~\cite{Pavlakos2017coarsefine} CVPR'17}
& 67.4 & 71.9 & 66.7 & 69.1 & 72.0 & 77.0 & 65.0 & 68.3 & 83.7 & 96.5 & 71.7 & 65.8 & 74.9 & 59.1 & 63.2 & 71.9 \\
\multicolumn{1}{l|}{Yoshiyasu \etal~\cite{DBLP:journals/corr/abs-1812-11328SkeletonTr} ACCV'18}
& 63.3 & 71.6 & 61.4 & 70.4 & 69.9 & 83.2 & 63.1 & 68.8 & 76.8 & 98.9 & 68.2 & 67.5 & 73.7 & 57.7 & 57.1 & 70.0 \\
\multicolumn{1}{l|}{Martinez \etal~\cite{DBLP:journals/corr/MartinezHRL17} ICCV'17} 
& 51.8 & 56.2 & 58.1 & 59.0 & 69.5 & 78.4 & 55.2 & 58.1 & 74.0 & 94.6 & 62.3 & 59.1 & 65.1 & 49.5 & 52.4 & 62.9 \\
\multicolumn{1}{l|}{Yang \etal~\cite{Yang18} CVPR'18}
& 51.5 & 58.9 & 50.4 & 57.0 & 62.1 & 65.4 & 49.8 & 52.7 & 69.2 & 85.2 & 57.4 & 58.4 & 43.6 & 60.1 & 47.7 & 58.6 \\ 
\multicolumn{1}{l|}{Chen \etal~\cite{Chen_2019_CVPR} CVPR'19}
& 45.9 &53.5 &50.1 &53.2 &61.5 &72.8 &50.7 &49.4 &68.4 &82.1 &58.6 &53.9 &57.6 &41.1 &46.0 &56.9  \\ 
\multicolumn{1}{l|}{Pavlakos \etal~\cite{pavlakos2018ordinal} CVPR'18}
& 48.5 & 54.4 & 54.4 & 52.0 & 59.4 & 65.3 & 49.9 & 52.9 & 65.8 & 71.1 & 56.6 & 52.9 & 60.9 & 44.7 & 47.8 & 56.2 \\
\multicolumn{1}{l|}{Luvizon \etal~\cite{Luvizon_2018_CVPR} CVPR'18}
& 49.2 & 51.6 & 47.6 & 50.5 & 51.8& 60.3 & 48.5 & 51.7 & 61.5 & 70.9 & 53.7 & 48.9 & 57.9 & 44.4 & 48.9 & 53.2 \\
\multicolumn{1}{l|}{Pavllo \etal~\cite{DBLP:PavLLO_3Dhumanposeinvideo} CVPR'19} 
& 47.1 & 50.6 & 49.0 & 51.8 & 53.6 & 61.4 & 49.4 & 47.4 &59.3 & 67.4 & 52.4 & 49.5 & 55.3 & \textbf{39.5} & 42.7 & 51.8 \\ \hline
\multicolumn{1}{l|}{Orientation keypoints (ours)} 
& 44.5 & 49.8 & 43.3 &46.4 &49.7 &52.0 &43.5 &44.4 &55.6 &64.7 &48.4 &45.3 &38.7 &50.1 &42.7 &47.9 \\
\multicolumn{1}{l|}{Refined orientation kps (ours)}
&\textbf{41.5} &\textbf{46.1} &\textbf{40.5} &\textbf{43.1} &\textbf{46.7} &\textbf{50.4} &\textbf{40.5} &\textbf{40.8} &\textbf{55.2} &\textbf{62.0} &\textbf{45.1} &\textbf{42.4} &\textbf{35.3} &\textbf{48.1} &\textbf{36.6} &\textbf{44.9} \\
\hline \\
\\
\textbf{Protocol \#2 (Procrustes)} & Dir & Disc & Eat & Greet & Phone & Photo & Pose & Punch & Sit & SitD & Smoke & Wait & WalkD & Walk & WalkT & Avg \\ \hline
\multicolumn{1}{l|}{Martinez \etal~\cite{DBLP:journals/corr/MartinezHRL17} ICCV'17} 
& 39.5 & 43.2 & 46.4 & 47.0 & 51.0 & 56.0 & 41.4 & 40.6 & 56.5 & 69.4 & 49.2 & 45.0 & 49.5 & 38.0 & 43.1 & 47.7 \\
\multicolumn{1}{l|}{Chen \etal~\cite{Chen_2019_CVPR} CVPR'19}

& 36.5 &41.0 &40.9 &43.9 &45.6 &53.8 &38.5 &37.3 &53.0 &65.2 &44.6 &40.9 &44.3 &32.0 &38.4 &44.1 \\
\multicolumn{1}{l|}{Pavlakos \etal~\cite{pavlakos2018ordinal} CVPR'18}
& 34.7 & 39.8 & 41.8 & 38.6 & 42.5 & 47.5 & 38.0 & 36.6 & 50.7 & 56.8 & 42.6 & 39.6 & 43.9 & 32.1 & 36.5 & 41.8 \\
\multicolumn{1}{l|}{Pavllo \etal~\cite{DBLP:PavLLO_3Dhumanposeinvideo} CVPR'19} 
& 36.0 & 38.7 & 38.0 & 41.7 & 40.1 & 45.9 & 37.1 & 35.4 & 46.8 & \textbf{53.4} & 41.4 & 36.9 & 43.1 & \textbf{30.3} & 34.8 & 40.0 \\ 
\multicolumn{1}{l|}{Yang \etal~\cite{Yang18} CVPR'18}
& \textbf{26.9} & \textbf{30.9} & 36.3 & 39.9 & 43.9 & 47.4 & \textbf{28.8} & \textbf{29.4} & \textbf{36.9} & 58.4 & 41.5 & \textbf{30.5} & 29.5 & 42.5 & 32.2 & 37.7 \\
\hline
\multicolumn{1}{l|}{Orientation keypoints (ours)} 
&33.8 &37.2 &35.3 &36.2 &37.2 &40.0 &33.3 &33.7 &43.0 &52.6 &37.3 &34.4 &30.6 &38.2 &33.6 &37.1\\ 
\multicolumn{1}{l|}{Refined orientation kps (ours)}
&32.2 &35.0  &\textbf{34.0}  &\textbf{34.7} &\textbf{36.1} &\textbf{39.0}  &31.7 &31.5 &42.9 &\textbf{50.3} &\textbf{36.3} &33.0  &\textbf{27.8} &37.1 &\textbf{30.6} &\textbf{35.5}\\
\hline \\
\end{tabular}%
}
\caption{Reconstruction error (mm) on Human 3.6M for single frame RGB images without depth information.  Lower is better, best highlighted in bold.  Numbers taken from original papers.  Our first line results are positions predicted by fitting rotations from the detector to the average training skeleton.  Refined results are post the second stage refiner network.  We do not show results on different protocols, and exclude \cite{sun2018integral} (as their preprocessing utilizes depth/scale information)}
\label{tab:mpjpe-table}
\end{table*}


==> tables/rotation_results_imp.tex <==
\begin{table}[]
\centering
%\resizebox{\linewidth}{!}{
\begin{tabular}{lrr}
\hline
& \multicolumn{1}{r}{MPJAS} & \multicolumn{1}{r}{MAA} \\ \hline
Yoshiyasu \etal~\cite {DBLP:journals/corr/abs-1812-11328SkeletonTr} ACCV '18 &0.424  &86.5\%   \\
 - pelvis (root) only & 0.226 & 92.8\% \\ \hline
 Orientation Keypoints (ours)\\
 2D detections + PnP & 0.265  & 91.6\%   \\
 3D detections + SVD & 0.217  & 93.0\%   \\
 - pelvis (root) only & 0.149 & 95.2\% \\
 \hline
\end{tabular}%
%}
\caption{Rotation results on Human3.6M. We average the 15 free rotations in the typical 17 joint skeleton.  We convert \cite{DBLP:journals/corr/abs-1812-11328SkeletonTr} as they report on a different basis. Hands and feet not included in the average as not in typical skeleton used in research.  Low MPJAS (in radians) and high MAA (accuracy) is better.  }
\label{tab:rotation-results}
\end{table}

